Differentially Private Variational Autoencoders with Term-wise Gradient Aggregation

This paper studies how to learn variational autoencoders with a variety of divergences under differential privacy constraints. We often build a VAE with an appropriate prior distribution to describe the desired properties of the learned representations and introduce a divergence as a regularization term to close the representations to the prior. Using differentially private SGD (DP-SGD), which randomizes a stochastic gradient by injecting a dedicated noise designed according to the gradient's sensitivity, we can easily build a differentially private model. However, we reveal that attaching several divergences increase the sensitivity from O(1) to O(B) in terms of batch size B. That results in injecting a vast amount of noise that makes it hard to learn. To solve the above issue, we propose term-wise DP-SGD that crafts randomized gradients in two different ways tailored to the compositions of the loss terms. The term-wise DP-SGD keeps the sensitivity at O(1) even when attaching the divergence. We can therefore reduce the amount of noise. In our experiments, we demonstrate that our method works well with two pairs of the prior distribution and the divergence.

==> 011_related.tex <==
\subsection{Related Works}

For privacy preserving data releasing, a traditional approach is to ensure $k$-anonymity \cite{sweeney2002k} and its variants \cite{machanavajjhala2006diversity} \cite{li2007t}.
There are lots of anonymization algorithms for various types of datasets and privacy requirements \cite{lefevre2006mondrian,lefevre2005incognito,takahashi2013top}.
To actualize a privacy-preserving data synthesis, we focus on releasing the parameters of generative models, but not anonymized data.

Generative models under DP have been studied in a last decade.
Traditional approaches are based on capturing probabilistic models, low rank structure, and learning statistical characteristics from original sensitive database \cite{zhang2014privbayes, zhang2017privbayes,chen2015differentially,zhang2016privtree}.
Plausible deniability \cite{bindschaedler2017plausible} is an extended privacy metric behind DP for building a generative model.
Due to well compress the data, we focus on building deep generative models, especially VAEs, under DP.


